Online Ride-Hitching in UAV Travelling

The unmanned aerial vehicle (UAV) has emerged as a promising solution to provide delivery and other mobile services to customers rapidly, yet it drains its stored energy quickly when travelling on the way and (even if solar-powered) it takes time for charging power on the way before reaching the destination. To address this issue, existing works focus more on UAV's path planning with designated system vehicles providing charging service. However, in some emergency cases and rural areas where system vehicles are not available, public trucks can provide more feasible and cost-saving services and hence a silver lining. In this paper, we explore how a single UAV can save flying distance by exploiting public trucks, to minimize the travel time of the UAV. We give the first theoretical work studying online algorithms for the problem, which guarantees a worst-case performance. We first consider the offline problem knowing future truck trip information far ahead of time. By delicately transforming the problem into a graph satisfying both time and power constraints, we present a shortest-path algorithm that outputs the optimal solution of the problem. Then, we proceed to the online setting where trucks appear in real-time and only inform the UAV of their trip information some certain time $\Delta t$ beforehand. As a benchmark, we propose a well-constructed lower bound that an online algorithm could achieve. We propose an online algorithm MyopicHitching that greedily takes truck trips and an improved algorithm $\Delta t$-Adaptive that further tolerates a waiting time in taking a ride. Our theoretical analysis shows that $\Delta t$-Adaptive is asymptotically optimal in the sense that its ratio approaches the proposed lower bounds as $\Delta t$ increases.

==> CHANGELOG <==
LIPICS Style - CHANGELOG

* 10/12/2018 LIPIcs-v2019 v2.0
** New Features
*** support of metadata in PDF file (e.g. author, title, keywords) 
*** revised displaying of author-related funding acknowledgements (now displayed as part of the funding block instead of footnotes)
*** added support for cleveref package (new document option 'cleveref')
*** added support for using autoref for theorem-like environments (new document option 'autoref')
*** added new environment claim and claimproof to realize sub-proofs
*** added new environment proposition
** Bugfixes
*** fixed problems with theorem-like environments when using cleveref and autoref (see new features above)
*** switched several URL from http to https
*** fixed problems with using of ACM 2012 classification (deactivated subjclass and revised support of ccsdesc macro)
** Minor changes
*** moved ORCID symbol behind author name (according https://orcid.org/content/journal-display-guidelines)
*** added separator \and to split several affiliations
*** added warnings when package 'enumitem' or 'paralist' are loaded; they manipulate the pre-defined enumeration styles and are partly incompatible
*** preloaded package 'microtype' in style
*** revised spacings/font sizes for top matter

* 09/04/2018 LIPIcs-v2018 v1.5
** Bugfixes
*** Fixed problem with page style in case of many authors
*** Fixed aggregation of authors for ToC file

* 15/03/2018 LIPIcs-v2018 v1.4
** Bugfixes
*** Fixed enumerations
*** Fixed aggregation of authors for ToC file

* 26/02/2018 LIPIcs-v2018 v1.3
** Bugfixes
*** Fixed \hideLIPIcs
*** Fixed enumerations
*** Fixed typo
** Revised display of ORCIDs following recommendation by ORCID

* 06/02/2018 LIPIcs-v2018 v1.2
** Release of LIPIcs-v2018
*** revised author macro \author{name}{affil}{email}{orcid}{funding} 
*** added support for ORCIDs
*** switched to ACM 2012 classification system
*** added new macros for extended metadata \category, \relatedversion, \supplement, \funding, \acknowledgements
*** added warnings for missing mandatory metadata
*** added preconfigured enumeration styles based on the enumerate package
*** added option \hideLIPIcs to hide all LIPIcs related information
*** added support for line numbers
** Bugfixes
*** fixed copyright line
*** added warning when using outdated subfig package due to incompatibilities in preloaded subcaption package
*** fixed bug when using MnSymbol package
*** fixed bug in numbering in theorem-like environments used in appendix
*** fixed problems in ToC file

